RCareWorld: A Human-centric Simulation World for Caregiving Robots

We present RCareWorld, a human-centric simulation world for physical and social robotic caregiving designed with inputs from stakeholders, including care recipients, caregivers, occupational therapists, and roboticists. RCareWorld has realistic human models of care recipients with mobility limitations and caregivers, home environments with multiple levels of accessibility and assistive devices, and robots commonly used for caregiving. It interfaces with various physics engines to model diverse material types necessary for simulating caregiving scenarios, and provides the capability to plan, control, and learn both human and robot control policies by integrating with state-of-the-art external planning and learning libraries, and VR devices. We propose a set of realistic caregiving tasks in RCareWorld as a benchmark for physical robotic caregiving and provide baseline control policies for them. We illustrate the high-fidelity simulation capabilities of RCareWorld by demonstrating the execution of a policy learnt in simulation for one of these tasks on a real-world setup. Additionally, we perform a real-world social robotic caregiving experiment using behaviors modeled in RCareWorld. Robotic caregiving, though potentially impactful towards enhancing the quality of life of care recipients and caregivers, is a field with many barriers to entry due to its interdisciplinary facets. RCareWorld takes the first step towards building a realistic simulation world for robotic caregiving that would enable researchers worldwide to contribute to this impactful field. Demo videos and supplementary materials can be found at: https://emprise.cs.cornell.edu/rcareworld/.

==> fig/representative.tex <==
 \begin{figure}[t!]
\centering
    \hfill
    \begin{subfigure}[h]{0.45\columnwidth}
		\centering
		  \framebox[\linewidth]{\raisebox{0}[0.5\linewidth][0]{{\small CareAvatars.}}}
	\end{subfigure}
	\hfill
	\begin{subfigure}[h]{0.45\columnwidth}
		\centering
		 \includegraphics[width=\linewidth]{fig/matterport.png}
	\end{subfigure}
	\hfill 
	\\
	\vspace{0.25cm}
	\begin{subfigure}[h]{\columnwidth}
		\centering
		  \includegraphics[width=0.99\linewidth]{fig/teaser.png}
	\end{subfigure}
    % \vspace{-0.25cm}
    \caption{We propose \textbf{RCareWorld}, a \textit{high-fidelity} human-centered simulation world for robotic caregiving.}
    \label{fig:teaser}
    \vspace{-0.8cm}
\end{figure}

==> sections/acknowledgement.tex <==
\section*{Acknowledgement}
This work was funded by the National Science Foundation IIS (\#2132846). 
